Super-CLEVR: A Virtual Benchmark to Diagnose Domain Robustness in Visual Reasoning

Visual Question Answering (VQA) models often perform poorly on out-of-distribution data and struggle on domain generalization. Due to the multi-modal nature of this task, multiple factors of variation are intertwined, making generalization difficult to analyze. This motivates us to introduce a virtual benchmark, Super-CLEVR, where different factors in VQA domain shifts can be isolated in order that their effects can be studied independently. Four factors are considered: visual complexity, question redundancy, concept distribution and concept compositionality. With controllably generated data, Super-CLEVR enables us to test VQA methods in situations where the test data differs from the training data along each of these axes. We study four existing methods, including two neural symbolic methods NSCL and NSVQA, and two non-symbolic methods FiLM and mDETR; and our proposed method, probabilistic NSVQA (P-NSVQA), which extends NSVQA with uncertainty reasoning. P-NSVQA outperforms other methods on three of the four domain shift factors. Our results suggest that disentangling reasoning and perception, combined with probabilistic uncertainty, form a strong VQA model that is more robust to domain shifts. The dataset and code are released at https://github.com/Lizw14/Super-CLEVR.

==> content/06_checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{} We work on diagnosis using synthetic dataset, which does include real data that may cause security issues; we do not introduce new models either. 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} In the sumpplementary material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} Because we are doing diagnosis on multiple dataset variants, where each model needs to be trained on different variants, so the cost for running multiple times is high. 
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}  We are evaluating existing methods and we include the training cost for high-cost method.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} In the supplementary material.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} The code for data generation and dataset examples are including in the supplemental material. The whole generated dataset is too large to attach.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} There is no data from other people.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{} Because the dataset is synthetic, it does not have personally identifiable information or offensive content.
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{} In the supplementary material.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{} 
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{} No participants are paid (excepts for cookies) because we only do a preliminary human study with a few annotators we know. 
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> content/TODO.tex <==


example in Fig1

caption of fig2

summary of results

motivation for part in intro

refine results

Code license in supplementary

==> content/a1_more_analysis.tex <==

\subsection{Part-based reasoning} \label{sec: part_results}

\textbf{Part-based questions.}
% In the CLEVR dataset, objects are simple, atomic shapes that can be referenced using holistic names or attributes. By contrast, in real-world data, objects are more complex and have hierarchical parts, which are studied in recent works \cite{liu2022learning, chen2014detect, hong2021ptr}. 
% Based on the intuition that a human may identify a specific object using its distinct parts, \eg ``the car with a shiny door'', in additional to object-based questions as in CLEVR, Super-CLEVR also include questions with hierarchical object parts. 


In addition to robustness diagnosing, Super-CLEVR can also be used to study part-based reasoning, since more complicated objects that has parts are already introduced into the scenes. We generate part-based questions that requires identifying objects with parts (\eg ``which vehicle has red door'') or querying about parts (\eg ``what color is the door of the car''). Examples of the part-based questions are shown in \cref{fig:part_example}.

To enable generation of part-based questions, we introduce two new operations in the reasoning program: \texttt{part\_to\_object($\cdot$)}, which find the objects containing the given part, and \texttt{object\_to\_part($\cdot$)}, which select all the parts of the given object. We also modify some of the existing operations (\ie \texttt{filter}, \texttt{query} and \texttt{unique}), enabling them to operate both on object-level and part-level. With those reasoning operations, we collect 9 part-based templates composed of the defined reasoning operations. Part-based questions are then generated by instantiating the templates with the image scene graph. 

\cref{tab: baseline_part} shows results of FiLM, mDETR and NSCL on part-based questions. First, all three methods perform poorly on part-based questions (less than 42\% accuracy), indicating the lack of ability to reason with hierarchical parts. This is consistent with the findings in \cite{hong2021ptr}. Second, among all models, mDETR performs best. This is possibly due to its ability to locate the small parts and the prior knowledge about object parts learned from pretraining. 

% FiLM gets 37.6\% accuracy on part questions, which is surprisingly good considering its relatively poor performance on object questions. We speculate that the strength of FiLM on part questions might come from its visual features: it relies on spatial features instead of mean-pooled object features, which gives it more potential to deal with small object parts. 

% The part-based result for NSCL is particularly low (25.93\%) compared to its superior performance on object questions, even though the groundtruth locations of each objects and parts, as well as the groundtruth reasoning programs, are provided to the model. Moreover, the speed of NSCL is very slow on part-based questions, which is due to the large number of part features. This suggests that the ROI-pooled features is not an optimal encoding for the parts, which are different from objects, indicating that the neural symbolic method studied here may need substantial improvements to handle part questions well.


\vspace{-0.2em}
\paragraph{Implementation details of part-based reasoning.} To enable reasoning with parts using the existing models, some minor modifications are needed. No change was made to FiLM; for mDETR and NSCL, the parts are treated the same way as objects. For mDETR, groundtruth bounding boxes of parts that appear in questions are provided to train the model; for NSCL, the concatenation of part and object features is fed into the model. All the models are trained with 200k object-based questions and 50k part-based questions. For FiLM and mDETR, the object and part questions are mixed and shuffled; for NSCL, the model is first pretrained with object questions only and then finetuned with part questions, due to the large number of part features.\footnote{It takes 8 days to train NSCL for 80 epochs on 50k part questions (multiple GPU does not help because bottleneck is the dense CPU operations in program execution).}

\begin{figure}[h]
\begin{center}
\vspace{-0.5em}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=1.0\linewidth]{figures/example.pdf}
\end{center}
    \vspace{-0.5em}
    \caption{Examples of part questions.}
\vspace{-1.5em}
\label{fig:part_example}
\end{figure}

\begin{table}[h]
\vspace{-0.25em}
\begin{center}
    % \begin{tabular}{lcc}
    % \toprule
    %     ~ & {\bf object} & \bf{part} \\ \midrule
    %     % {\bf Random} & 33.13 & 21.38 \\ 
    %     % {\bf Majority} & 40.69 & 22.75 \\ 
    %     % {\bf LSTM} & 46.34 & 20.93 \\ 
    %     % {\bf CNN+LSTM} & 48.87 & 24.57 \\ 
    %     {\bf FiLM} & 53.20 & 37.61 \\ 
    %     {\bf mDETR} & 82.65 & 41.32 \\ 
    %     {\bf NSCL} & 89.09 & 25.93 \\ 
    %     % \hline
    %     % Human & 66.30 & 59.85 \\ 
    % \bottomrule
    % \end{tabular}
    \begin{tabular}{lccc}
    \toprule
        {\bf ~} & {\bf FiLM} & \bf{mDETR} & \bf{NSCL}\\ 
        \midrule
        {\bf Acc.} & 37.61 & 41.32 & 25.93 \\
    \bottomrule
    \end{tabular}
\end{center}
\vspace{-1.5em}
\caption{Models' accuracy on part-based questions.}
\label{tab: baseline_part}
\vspace{-0.5em}
\end{table}
